Models of force-free spheres and applications to solar active regions

Here we present a systematic study of force-free field equation for simple axisymmetric configurations in spherical geometry. The condition of separability of solutions in radial and angular variables leads to two classes of solutions: linear and non-linear force-free fields. We have studied these linear solutions Chandrasekhar (1956) and extended the non-linear solutions given in Low \& Lou (1990) to the irreducible rational form $n= p/q$, which is allowed for all cases of odd $p$ and to cases of $q>p$ for even $p$. We have further calculated their energies and relative helicities for magnetic field configurations in finite and infinite shell geometries. We demonstrate here a method here to be used to fit observed magnetograms as well as to provide good exact input fields for testing other numerical codes used in reconstruction on the non-linear force-free fields.

==> def.tex <==
\let\new=\newcommand
\new{\be}{\begin{equation}}
\new{\ee}{\end{equation}}
\new{\disp}{\displaystyle}
\new{\bdm}{\begin{displaymath}}
\new{\edm}{\end{displaymath}}
\new{\bi}{\begin{itemize}}
\new{\ei}{\end{itemize}}
\new{\ben}{\begin{enumerate}} 
\new{\een}{\end{enumerate}}
\new{\bfig}{\begin{figure}}
\new{\efig}{\end{figure}}
\new{\bea}{\begin{eqnarray*}}
\new{\eea}{\end{eqnarray*}}
\new{\RHO}{\mbox{\boldmath $\rho$}}
\new{\ZETA}{\mbox{\boldmath $\zeta$}}
\new{\PI}{\mbox{\boldmath $\Pi$}}
\new{\OMEGA}{\mbox{\boldmath $\omega$}}
\new{\B}{{\bf B}}
\new{\vel}{{\bf v}}
\new{\vb}{{\bf b}}
\new{\av}{{\bf a}}
\new{\cv}{{\bf c}}
\new{\kv}{{\bf k}}
\new{\K}{{\bf K}}
\new{\xv}{{\bf x}}
\new{\uv}{{\bf u}}
\new{\wv}{{\bf w}}
\new{\hv}{{\bf h}}
\new{\X}{{\cal X}}
\new{\T} {{\cal T}}
\new{\E}{{\bf E}}
\new{\je}{{\bf j_e}}
\new{\jv}{{\bf j}}
\new{\ol}{\overline}
\new{\curl}{ \nabla \times}
\new{\Div}{ \nabla \cdot}
\new{\lap}{\nabla^2}
\new{\del}{\partial}
\new{\nor}{\nabla \chi}
% \newfont{\zf}{ZapfChancery-MediumItalic scaled 1500}
% \new{\rs}{{\hbox{\zf r}}}
% \newfont{\bigbo}{Times-Roman scaled 2000}
% \newfont{\typo}{Times-Roman  scaled 1500}

